Depth Pro 2: Sharp and Temporally Consistent Metric Monocular Depth

We present Depth Pro 2, an approach to estimating dense metric depth for images and video at full resolution. By analyzing prior methods for monocular depth estimation, we find that they commonly trade off temporal consistency and boundary sharpness: multi-frame methods favor consistency, single-frame methods favor sharpness. To overcome this trade-off, we train a single, scalable network that processes both images and video and predicts depth maps at native resolution. Depth Pro 2 produces depth maps that are metrically accurate, sharp, and temporally consistent all at once, outperforming prior work in all of these dimensions. We release a family of models that define a new Pareto frontier in terms of metric accuracy, sharpness, temporal consistency, and runtime. We release code and weights at https://apple-aiml-research.github.io/ml-depth-pro-2/

==> tex/figures/qualgrid.tex <==
\ifdefined\qualfigure\expandafter\endinput\fi
\makeatletter

\newcommand{\qualdir}{figures/qualitative_sharpness}

\newcommand{\example}[6]{%
  \expandafter\gdef\csname qual@stem@#1\endcsname{#2}%
  \expandafter\gdef\csname qual@box@#1\endcsname{\def\qx{#3}\def\qy{#4}\def\qX{#5}\def\qY{#6}}}
\newcommand{\methods}[1]{\def\qual@methods{#1}}

\pgfkeys{/qual/.is family, /qual,
  rows/.store in=\qual@rows,          zoom/.store in=\qual@zoom,
  wrap/.store in=\qual@wrap,
  width/.store in=\qual@width,        height/.store in=\qual@height,
  gap/.store in=\qual@gap,            zoom gap/.store in=\qual@zoomgap,
  row gap/.store in=\qual@rowgap,     column gap/.store in=\qual@colgap,
  inset/.store in=\qual@inset,        inset margin/.store in=\qual@insetm,
  box color/.store in=\qual@boxcolor, box width/.store in=\qual@boxw,
  box outline/.store in=\qual@outline, box outline width/.store in=\qual@outlinew,
  box style/.code={\tikzset{qual dash/.style={#1}}},
  box opacity/.store in=\qual@opacity, zoom border/.store in=\qual@zoomborder,
  zoom border methods/.store in=\qual@zbmethods,
  zoom border outline/.store in=\qual@zbo,
  zoom border outline width/.store in=\qual@zbow,
  zoom border width/.store in=\qual@zbw,
  zoom border color/.store in=\qual@zbc,
  crop top/.store in=\qual@croptop,
  label font/.store in=\qual@labelfont, label width/.store in=\qual@labelw}
\newcommand{\qualset}[1]{\pgfkeys{/qual,#1}}
\qualset{rows=examples, zoom=below, wrap=0, width=\linewidth, height=0.9\textheight,
  gap=1.5pt, row gap={}, column gap={}, zoom gap=0.5pt, inset=0.4, inset margin=0pt,
  box color=white, box width=0.4pt, box outline=black, box outline width=1pt,
  box style=solid, box opacity=1, zoom border=false, zoom border methods={},
  zoom border outline={}, zoom border outline width={}, zoom border width={},
  zoom border color={}, crop top=0,
  label font=\sffamily\scriptsize, label width=9pt}

\qualset{qual lines/.style={box color=qualbox, box outline width=0pt,
  zoom border outline=none, zoom border width=1pt}}

\ExplSyntaxOn
\NewDocumentCommand \qual@foreach { m m }
  { \clist_set:Nx \l_tmpa_clist {#1} \clist_map_inline:Nn \l_tmpa_clist { \def\qe{##1} #2 } }

\NewDocumentCommand \qual@zbtest { m }
  {
    \clist_set:Nx \l_tmpa_clist { \qual@zbmethods }
    \tl_set:Nx \l_tmpb_tl {#1}
    \clist_if_empty:NTF \l_tmpa_clist
      { \str_if_eq:eeTF { \qual@zoomborder } { true } { \qual@zbtrue } { \qual@zbfalse } }
      { \clist_if_in:NVTF \l_tmpa_clist \l_tmpb_tl { \qual@zbtrue } { \qual@zbfalse } }
  }
\ExplSyntaxOff
\newif\ifqual@zb

\def\qual@img#1#2{\includegraphics[#1]{#2}}
\def\qual@is#1#2{\edef\qual@a{#1}\def\qual@b{#2}\ifx\qual@a\qual@b}
\newsavebox\qual@probe
\newbox\qual@grid \newbox\qual@row \newbox\qual@heads
\newcount\qual@n \newcount\qual@k
\newlength\qual@len
\newif\ifqual@first

\def\qual@open#1#2{%
  \edef\qfile{\qualdir/\csname qual@stem@#1\endcsname_#2}%
  \sbox\qual@probe{\qual@img{}{\qfile}}%
  \edef\qaF{\fpeval{\ht\qual@probe/\wd\qual@probe}}%
  \edef\qa{\fpeval{\qaF*(1-\qual@croptop)}}%
  \csname qual@box@#1\endcsname
  \edef\qb{\fpeval{(\qY-\qy)*\qaF/(\qX-\qx)}}}

\def\qual@shape{%
  \edef\qual@alpha{1}\edef\qual@beta{0}\edef\qual@gamma{\qa}\edef\qual@delta{0}%
  \qual@is\qual@zoom{below}\edef\qual@gamma{\fpeval{\qa+\qb}}\edef\qual@delta{\fpeval{\qual@zoomgap}}\fi
  \qual@is\qual@zoom{right}\edef\qual@alpha{\fpeval{1+\qa/\qb}}\edef\qual@beta{\fpeval{\qual@zoomgap}}\fi}

\def\qual@stroke#1{%
  \qual@is\qual@outline{none}\else
    \draw[qual dash, line width=\qual@outlinew, draw=\qual@outline, draw opacity=\qual@opacity] #1;
  \fi
  \draw[qual dash, line width=\qual@boxw, draw=\qual@boxcolor, draw opacity=\qual@opacity] #1;}

\def\qual@bands#1#2#3#4{%
  \edef\qzoc{\qual@outline}\qual@is\qual@zbo{}\else\edef\qzoc{\qual@zbo}\fi
  \edef\qzow{\qual@outlinew}\qual@is\qual@zbow{}\else\edef\qzow{\qual@zbow}\fi
  \edef\qzcw{\qual@boxw}\qual@is\qual@zbw{}\else\edef\qzcw{\qual@zbw}\fi
  \edef\qzcc{\qual@boxcolor}\qual@is\qual@zbc{}\else\edef\qzcc{\qual@zbc}\fi
  \edef\qzo{0}%
  \qual@is\qzoc{none}\else
    \edef\qzo{\fpeval{\qzow}}%
    \draw[qual dash, line width=\qzow, draw=\qzoc, draw opacity=\qual@opacity]
      (\fpeval{#1+\qzo/2},\fpeval{#2+\qzo/2})
      rectangle ++(\fpeval{#3-\qzo},\fpeval{#4-\qzo});
  \fi
  \edef\qzc{\fpeval{\qzcw}}%
  \draw[qual dash, line width=\qzcw, draw=\qzcc, draw opacity=\qual@opacity]
    (\fpeval{#1+\qzo+\qzc/2},\fpeval{#2+\qzo+\qzc/2})
    rectangle ++(\fpeval{#3-2*\qzo-\qzc},\fpeval{#4-2*\qzo-\qzc});}

\def\qual@cell#1#2#3{%
  \begingroup
  \qual@open{#1}{#2}%
  \edef\qW{#3}\edef\qH{\fpeval{#3*\qa}}\edef\qm{\fpeval{\qual@insetm}}%
  \edef\qzw{\fpeval{\qual@inset*\qW}}\edef\qzh{\fpeval{\qzw*\qb}}%
  \edef\qzx{\fpeval{\qm}}\edef\qzy{\fpeval{\qH-\qm-\qzh}}%
  \qual@is\qual@zoom{top right}\edef\qzx{\fpeval{\qW-\qm-\qzw}}\fi
  \qual@is\qual@zoom{bottom left}\edef\qzy{\qm}\fi
  \qual@is\qual@zoom{bottom right}\edef\qzx{\fpeval{\qW-\qm-\qzw}}\edef\qzy{\qm}\fi
  \qual@is\qual@zoom{below}%
    \edef\qzw{\qW}\edef\qzh{\fpeval{\qW*\qb}}\edef\qzx{0}\edef\qzy{\fpeval{-\qual@zoomgap-\qzh}}\fi
  \qual@is\qual@zoom{right}%
    \edef\qzh{\qH}\edef\qzw{\fpeval{\qH/\qb}}\edef\qzx{\fpeval{\qW+\qual@zoomgap}}\edef\qzy{0}\fi
  \begin{tikzpicture}[x=1pt, y=1pt]
    \path[use as bounding box] (0,\fpeval{min(0,\qzy)}) rectangle (\fpeval{max(\qW,\qzx+\qzw)},\qH);
    \node[anchor=south west, inner sep=0pt, outer sep=0pt] at (0,0)
      {\qual@img{trim={0 0 0 {\qual@croptop\ht\qual@probe}}, clip, width=\qW pt}{\qfile}};
    \node[anchor=south west, inner sep=0pt, outer sep=0pt] at (\qzx,\qzy)
      {\qual@img{trim={\qx\wd\qual@probe} {\fpeval{1-\qY}\ht\qual@probe}
                        {\fpeval{1-\qX}\wd\qual@probe} {\qy\ht\qual@probe},
                  clip, width=\qzw pt}{\qfile}};
    \qual@stroke{(\fpeval{\qW*\qx},\fpeval{\qW*\qaF*(1-\qY)}) rectangle (\fpeval{\qW*\qX},\fpeval{\qW*\qaF*(1-\qy)})}
    \qual@zbtest{#2}\ifqual@zb
      \qual@bands{\qzx}{\qzy}{\qzw}{\qzh}%
    \fi
  \end{tikzpicture}%
  \endgroup}

\def\qual@rowlabel#1#2{%
  \hbox to \qual@labelw{\hss\rotatebox{90}{\hbox to #2pt{\hss\qual@labelfont #1\hss}}\hss}}
\def\qual@head#1#2{\hbox to #2pt{\hss\qual@labelfont\strut #1\hss}}
\def\qual@emit#1{\ifqual@first\qual@firstfalse\else\vskip\qual@rgap\fi\box#1}
\def\qual@append#1#2{\setbox#1=\hbox{\ifvoid#1\else\unhbox#1\hskip\qual@cgap\fi#2}}

\def\qual@solve#1{%
  \qual@n=0 \def\method##1##2{\advance\qual@n 1 \ifnum\qual@n=1 \def\qfirst{##1}\fi}\qual@methods
  \edef\qM{\the\qual@n}\edef\qN{0}\edef\qS{0}%
  \qual@foreach{#1}{%
    \qual@open\qe\qfirst\qual@shape
    \edef\qN{\the\numexpr\qN+1}%
    \qual@is\qual@rows{methods}\edef\qS{\fpeval{\qS+\qual@alpha/\qual@gamma}}%
    \else\edef\qS{\fpeval{\qS+\qual@gamma/\qual@alpha}}\fi}%
  \setlength\qual@len{\qual@width}\edef\qT{\fpeval{\qual@len}}%
  \setlength\qual@len{\qual@height}\edef\qU{\fpeval{\qual@len}}%
  \setbox0\hbox{\qual@labelfont\strut}\edef\qhh{\fpeval{\ht0+\dp0}}%
  \qual@is\qual@rows{methods}%
    \edef\qp{\fpeval{min(
      (\qT-\qual@labelw-\qN*(\qual@cgap+\qual@beta)+\qS*\qual@delta)/\qS,
      (\qU-(\qM-1)*\qual@rgap)/\qM)}}%
  \else
    \edef\qC{\ifnum\qual@wrap>0 \qual@wrap\else\qM\fi}%
    \edef\qR{\fpeval{ceil(\qM/\qC)}}%
    \edef\qheads{\ifnum\qual@wrap>0 \fpeval{\qN*\qR}\else 1\fi}%
    \edef\qp{\fpeval{min((\qT-(\qC-1)*\qual@cgap)/\qC,
      (\qU-\qheads*\qhh-(\qN*\qR+\qheads-1)*\qual@rgap-\qN*\qR*\qual@delta)/(\qR*\qS)
        +\qual@beta)}}%
  \fi
  \qual@foreach{#1}{%
    \qual@open\qe\qfirst\qual@shape
    \qual@is\qual@rows{methods}\edef\qw{\fpeval{(\qp-\qual@delta)/\qual@gamma}}%
    \else\edef\qw{\fpeval{(\qp-\qual@beta)/\qual@alpha}}\fi
    \expandafter\xdef\csname qual@W@\qe\endcsname{\qw}}}

\def\qual@W#1{\csname qual@W@#1\endcsname}

\def\qual@methodrow#1#2{%
  \def\qmf{#1}%
  \setbox\qual@row=\hbox{\qual@rowlabel{#2}{\qp}}%
  \qual@foreach{\qual@list}{\qual@append\qual@row{\qual@cell\qe\qmf{\qual@W\qe}}}%
  \qual@emit\qual@row}

\def\qual@examplerow{%
  \qual@k=0
  \let\method\qual@examplecell
  \qual@methods
  \ifnum\qual@k>0 \qual@flush\fi}
\def\qual@examplecell#1#2{%
  \qual@append\qual@heads{\qual@head{#2}{\qp}}%
  \qual@append\qual@row{\qual@cell\qe{#1}{\qual@W\qe}}%
  \advance\qual@k 1
  \ifnum\qual@k=\qC\relax\qual@flush\fi}

\def\qual@flush{%
  \ifnum\qual@wrap>0 \qual@emit\qual@heads
  \else\ifqual@first\qual@emit\qual@heads\else\setbox\qual@heads=\box\voidb@x\fi\fi
  \qual@emit\qual@row
  \qual@k=0 }

\NewDocumentCommand\qualfigure{o m}{%
  \begingroup
  \IfValueT{#1}{\qualset{#1}}%
  \edef\qual@rgap{\qual@rowgap}\qual@is\qual@rowgap{}\edef\qual@rgap{\qual@gap}\fi
  \edef\qual@cgap{\qual@colgap}\qual@is\qual@colgap{}\edef\qual@cgap{\qual@gap}\fi
  \def\qual@list{#2}%
  \qual@solve\qual@list
  \qual@firsttrue
  \setbox\qual@grid=\vbox{\offinterlineskip
    \qual@is\qual@rows{methods}\let\method\qual@methodrow\qual@methods
    \else\qual@foreach{\qual@list}{\qual@examplerow}\fi}%
  \leavevmode\box\qual@grid
  \endgroup}

\makeatother

